Towards Generalizable Reinforcement Learning for Trade Execution

Optimized trade execution is to sell (or buy) a given amount of assets in a given time with the lowest possible trading cost. Recently, reinforcement learning (RL) has been applied to optimized trade execution to learn smarter policies from market data. However, we find that many existing RL methods exhibit considerable overfitting which prevents them from real deployment. In this paper, we provide an extensive study on the overfitting problem in optimized trade execution. First, we model the optimized trade execution as offline RL with dynamic context (ORDC), where the context represents market variables that cannot be influenced by the trading policy and are collected in an offline manner. Under this framework, we derive the generalization bound and find that the overfitting issue is caused by large context space and limited context samples in the offline setting. Accordingly, we propose to learn compact representations for context to address the overfitting problem, either by leveraging prior knowledge or in an end-to-end manner. To evaluate our algorithms, we also implement a carefully designed simulator based on historical limit order book (LOB) data to provide a high-fidelity benchmark for different algorithms. Our experiments on the high-fidelity simulator demonstrate that our algorithms can effectively alleviate overfitting and achieve better performance.

==> inputs/app_algo.tex <==
\begin{algorithm}[H]
\caption{CASH: Context Aggregation with Handcrafted Statistics}
\label{algo:CASH_full}
\begin{algorithmic}[1]
\STATE Initialize context encoder $\phi_{\theta}(\cdot)$, PolicyNet/ValueNet $\text{RL}_{w}(\cdot,\cdot)$;
\STATE Given hand-crafted statistics function $\phi_{\text{hand}}(\cdot)$, Simulated Environment $E$;

\STATE \textit{\# Pre-train the context encoder}
\FOR{$i = 1 $ \textbf{to} $ n$}
    \STATE Sample minibatch $\{(c_{j}, {c'}_{j})\}$ from simulator $E$ with arbitrary actions;
    \STATE Using gradient descent to minimize the loss $ \mathcal{L}_\text{stat}(\theta)= \sum_{j} (\phi_{\theta}(c_{j}) - \phi_{\text{hand}}({c'}_{j}))^{2}$;
\ENDFOR
\STATE \textit{\# Train the RL model}
\STATE Fix the parameters $\theta$ in the context encoder $\phi_{\theta}(\cdot)$;
\FOR{$i = 1 $ \textbf{to} $m$}
    \STATE Sample minibatch $\{(c_{j}, {s}_{j}, r_{j})\}$ from simulator $E$ by rolling the current policy;
    \STATE Train $\text{RL}_{w}(\phi_{\theta}(c_{j}), s_{j})$ by minimizing loss $\mathcal{L}(w)=\sum_{j} \mathcal{L}_\text{RL}(w)$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{CATE}
\label{algo:CATE_full}
\begin{algorithmic}[1]
\STATE Initialize context encoder $\phi_{\theta}(\cdot)$, future encoder $\phi_{\vartheta}(\cdot)$, PolicyNet/ValueNet $\text{RL}_{w}(\cdot,\cdot)$;
\STATE Given simulator $E$;

\STATE \textit{\# Train model simultaneously in an end-to-end manner}
\FOR{$i = 1 $ \textbf{to} $ m$}
    \STATE Sample minibatch $\{(c_{j}, {c}_{j}')\}$ from simulator $E$ by rolling the current policy;
    \STATE Using gradient descent to minimize the loss 
    \[
    \mathcal{L}(\theta, \vartheta, w):= \sum_{j} \mathcal{L}_{\text{Enc}}(\theta, \vartheta) + \mathcal{L}_{\text{RL1}}(\theta, w) + \mathcal{L}_{\text{RL2}}(\vartheta, w)
    \]
\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\caption{Simulator}
\label{algo:simulation}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Policy $\pi$, 
\STATE \textbf{Given:} Historical dataset $D$, transition dynamics $P(s'|c,s,a)$, and reward function $r(c,s,a)$, execution period $T$, and execution volume $V$;
\STATE Pick a context trajectory $\{c_1, c_2, \cdots, c_T\}$ from $D$;
\STATE Initialize $s_1$ and output $(c_1,s_1)$
\FOR{$t = 1 $ \textbf{to} $ T$}
    \STATE Receive an action $a_t$ from $\pi$;
    \STATE Calculate $s_{t+1} \sim P(\cdot|c_t, s_t, a_t)$ and $r_{t} = r(c_t, s_t, a_t)$;
    \STATE Return $(r_t, c_{t+1}, s_{t+1})$;
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> inputs/app_experiments.tex <==
\textbf{Toy trade execution task.}
The reward in the toy trade execution task is $r=(\sum_{t=31}^{60} \gamma^{t-31} a_t p_t) - (\frac{1}{30} \sum_{t=31}^{60} \gamma^{t-31} p_t)$, where $a_t$ is the action, $p_t$ is the price, and we set $\gamma=\exp(\log(\frac{1}{2}) / 30)= 0.9772$.
We present more results on the learned strategy by ``RL'' and ``Fit parameters'' for the toy trade execution task to illustrate how an overfitted/generalizable policy should perform.
We present their performance under different market environments in Figure \ref{fig:toy}.
In general, when the price is rising (see the left two columns in the figure), a good strategy should sell more at the end of the horizon; otherwise (see the right two columns) a good strategy needs to liquidate as soon as possible. 
Moreover, ``RL'' presents sharp peaks which indicates that it suffers from overfitting the training data while ``Fit parameters'' liquidates the inventory smoothly and resembles the analytical solution in previous papers \cite{almgren2001optimal}.

\begin{figure*}[t]
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{inputs/fig_RL_1k.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{inputs/fig_fit_param_1k.png}
     \end{subfigure}
     \caption{The static strategy learned by ``RL'' (top) and ``Fit parameters'' (bottom). The blue lines are the prices and the orange lines are the trading rates determined by the strategies. 
The price sequences in the five figures from left to right are generated using $\sigma=1.5$ and $\alpha=1.0, 0.5, 0.0, -0.5, -1.0$ respectively.}
     \label{fig:toy}
\end{figure*}

\textbf{Ablation study on the model designs for trade execution.}
We conduct experiments on the combination of the designs on the observation space, reward function, learning rate, model architecture, etc.
We perform a grid search over all the possible combinations and list the corresponding performance impacts in Table \ref{tab:ablation}.
We can observe that the most influential factor is the design in the reward function.
Tuned DQN/PPO and Algo1/Algo2 use the design that is the best in each group.
\input{inputs/tab_ablation.tex}

We conduct a grid search over all possible designs listed in the table and run each combination five times. 
We show the differences between the average trading cost when the model adopts the design and the average trading cost over the runs in the whole set.
For the first group, the whole set contains all runs for tuned PPO.
For the second to the fifth group, the whole set only contains runs for tuned PPO that use \emph{cash inflow} as the revenue term.
For the last group, the whole set contains all runs for Algo1 (PPO).
\begin{itemize}
\item Equally distributed quoted volumes ranges from 0 to 2TWAP as is in \cite{daberius2019deep}.
\item The quoted price is selected from a non-uniformly distributed set $P$=[[-50, -40, -30, -25, -20, -15], linspace(-10, 10, 21), [15, 20, 25, 30, 40, 50]] bp.
\item The quoted price and volume is selected from $[\frac{1}{2}\text{TWAP}, \text{TWAP}, \frac{3}{2}\text{TWAP}, 2 \text{TWAP}] \times P$.
\end{itemize}





\textbf{Increasing the data volume.}
We argue that simply increasing the data volume does not address the overfitting problem since the RL agents are trained in the low-data region in practice.
Although there is a large amount of historical data available in finance, the high noise and high dimensionality of the context (i.e., the indicators) calls for far more samples than we have.
Moreover, in real trading, although using far data augments the dataset, this may also induce the distribution shift due to the fast changing market environment.
To validate our claim, we conduct new experiments using more data (6 months $\approx 3$M samples) and compare them with our main experiment. 
We present the result in Table \ref{tab:more_data}.
We observe that simply using more data does not alleviate overfitting and our algorithm achieves better performance when more data is consumed.

\begin{table}[htbp]
\tiny
\centering
\begin{tabular}{ r r r r}
Algorithm & Training & Testing & Gap \\
\hline
tuned DQN (2 months) & 1.6078 (2.1974) & 6.7199 (2.7776) & 5.1121 \\ 
tuned DQN (6 months) & 2.0545 (2.8511) & 6.1737 (2.3555) & 4.1192 \\ 
CATE+DQN (2 months) & -2.7526 (1.3319) & 0.0749 (1.5233) & 2.8275 \\ 
CATE+DQN (6 months) & -3.0444 (1.8510) & 0.7940 (0.5523) & 3.8384 \\ 
\end{tabular}
\caption{Performance of the RL agents trained using more data. The experiment setting is the same as the setting in Table \ref{tab:main_exp}.}
\label{tab:more_data}
\end{table}


\textbf{Hardware.}
Our experiments are conducted on a server with the following configurations:
\begin{itemize}
    \item System: Ubuntu 18.04.5 LTS
    \item CPU: 24 x Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz
    \item GPU: 4 x Tesla V100
    \item Memory: 441G
\end{itemize} 

\textbf{Limitation and social impact of our work.}
Generalization in trade execution or other tasks in quantitative investment is important. This paper only studies on how to improve generalization from the representation learning perspective. There are other aspects that are worth investing such as feature engineering, neural architecture design, and traditional deep learning techniques that can prevent overfitting.
Trade execution is an important application in the financial industry.
With a good trade execution strategy, the firms can allocate the resources more efficiently.

% We argue that overfitting in trade execution could happen ``robustly`` even if we use a reasonably large offline dataset.
% Notice that overfitting happens in our main experiments (cf. Table \ref{tab:main_exp}) where the trading frequency is high and the training already consumes a large amount of data (with approximately 1 million samples).
% To compare with

% We conduct new experiments using more data (6 months $\approx 3$M samples) and present the results as follows. We can see that simply using more data does not alleviate overfitting. 
% 股票数量特别多，高频的数据，数据量已经很大了。datasize 超出了 daily based 的二十年的数据。




==> inputs/app_lob.tex <==
We present an LOB snapshot of one stock in Table \ref{table:LOB} which consists of five levels of the ask/bid prices and volumes.
\emph{Ask/bid prices and volumes} indicate that there are specific volumes of stock to sell/buy at the specified prices.
The first level of ask/bid price (i.e., the lowest ask price or the highest bid price) is referred to as \emph{the best ask/bid price}.
The \emph{mid price} is the average of the best ask price and the best bid price, and the \emph{spread} is the gap between them.
For example, the mid price is $(\$29.11 + \$29.01) / 2 = \$29.06$ and the spread is $\$29.11-\$29.01=\$0.10$ on the given snapshot.
The traders can trade via two types of orders: market orders (MOs) and limit orders (LOs).
An MO specifies the volume and is executed immediately with the best available price.
For example, an MO that sells $500$ shares of the stock will be executed at the average price $(\$29.01 \times 100 + \$29.00 \times 300 + \$28.99 \times 100) / 500 = \$29.00$. 
We observe that the average execution price is lower than the mid price, and the gap $\$29.06 - \$29.00=\$0.06$ is referred to as the \emph{temporary market impact}.
An LO specifies the volume as well as the price such that the trader will buy/sell the asset with a price no higher/lower than the preset price.
If LO is not executed immediately, it will be left in the LOB and appended to the order queue on the corresponding price level. 

\begin{table}[tbhp]
\centering
\begin{tabular}{ crr  }
 & Price & Volume \\
 \hline
 Ask 5 & \$29.15 & 10,000 \\
 Ask 4 & \$29.14 & 2,000 \\
 Ask 3 & \$29.13 & 1,000 \\
 Ask 2 & \$29.12 & 100 \\
 Ask 1 & \$29.11 & 200 \\
 \hline
 Bid 1 & \$29.01 & 100 \\
 Bid 2 & \$29.00 & 300 \\
 Bid 3 & \$28.99 & 800 \\
 Bid 4 & \$29.95 & 1,100 \\
 Bid 5 & \$29.09 & 1,900 \\
 \hline
\end{tabular}
\vspace{0.5cm}
\caption{A snapshot of the limit order book.}
\label{table:LOB}
\end{table}

==> inputs/app_novelty.tex <==
We believe the overfitting problem in ORDC is novel.
Most existing papers study the setting where the agent is trained and evaluated on different sets of seeds/configurations [1-3] or procedurally generated environments [4-7].
ORDC is different from their settings in that 1) the context changes in each time step and affects both the reward and the transition; 2) the context sequence is highly stochastic and pre-collected with limited samples.
These properties contribute to the high variance in estimating $Q(c,s,a)$~(cf. Figure 5) and thus exacerbate overfitting.
% \li{All these properties contribute to the high variance in value estimation for $Q(c,s,a)$~(Figure.5), therefore leads to the overfitting issue.}
Moreover, ORDC is worth studying since it generalizes many industrial applications.
For example, the context can be the customer/electricity demand in inventory/power grid management or the incoming tasks for ride-sharing tasks.
Thus, the analysis and the methods in our paper can also be applied to these domains.
Besides, 
few papers (if any) mention the idea to aggregate the context/state space,
% the idea to aggregate the context/state is mentioned by few papers,
and our approach that aggregates the context space by predicting future context statistics is different from existing state abstraction methods (e.g., predicting the future reward/transition/return).

Since the market status sequence is collected offline, we believe the proposed ORDC framework can provide a better tool to analyze the overfitting problem (which is a key challenge in finance) compared with the standard MDP formulation used in most existing finance papers.
As for our methods, 
while the previous study suggests feature engineering, CATE goes a step further to generate features automatically. The latent factor model in finance is not used to prevent overfitting in the machine learning context.

==> inputs/app_proof1.tex <==
The proof of the lower bound mainly follows \cite{azar2013minimax} which studies the standard MDP.
First, we construct a class of ORDC models $\mathbb{M}$.
Then, following the analysis in \cite{azar2013minimax}, we can obtain the result that any algorithm in a subset of algorithms $A \in \mathfrak{A}' \subset \mathfrak{A}$ can fail to learn an accurate value function for at least one of the models in $\mathbb{M}$ with a high probability if the context dataset is not large enough.
At last, we generalize this conclusion to any of the possible algorithms $A\in\mathfrak{A}$ by showing that we can always find an algorithm $A'\in\mathfrak{A}'$ that performs no worse than $A$.

\begin{proof}
We first define a class of ORDC models $\mathbb{M}$.
For each instance $M$ in the class, the reward depends only on the context, i.e., $r(c,s,a)=r(c)$.
The context space is divided into three disjoint subsets of equal cardinality, i.e., $\mathcal{C} = \mathcal{C}^0 \cup \mathcal{C}^1 \cup \mathcal{C}^2$, $|\mathcal{C}|=3K$, and $|\mathcal{C}^0|=|\mathcal{C}^1|=|\mathcal{C}^2|=K$.
For each context in $c^0 \in \mathcal{C}^0$, it will trainsit to the corresponding context $c^1 \in \mathcal{C}^1$ with probability 1.
For each context $c^1 \in \mathcal{C}^1$, it will transit to the corresponding context $c^2 \in \mathcal{C}^2$ with probability $1-p_M$ and to itself with probability $p_M$.
For each context $c^2 \in \mathcal{C}^2$, it will transit to itself with probability 1.
The transition probability $p_M$ for each $c\in\mathcal{C}^1$ is selected from $\{p, p+\alpha\}$, where $\alpha$ and $p$ satisfy $0<p<p+\alpha<1$, and the exact value is determined in the analysis.
The reward function is 
\begin{equation}
    r(c) = \begin{cases}
    1 & \text{if } c\in \mathcal{C}^1 \\
    0 & \text{otherwise}
    \end{cases}.
\end{equation}
It is not hard to see that $Q_M^*(c,s,a)=\frac{\gamma}{1-\gamma p_M} =: \mathbb{Q}_M^*(c), \forall c\in\mathcal{C}^0$.
% Now, let us consider two ORDC models $M_1$ and $M_2$ with the transition probability $p_M$ equals to $p$ and $p+\alpha$ respectively, where $\alpha$ and $p$ satisfies that $0<p<p+\alpha<1$ and the exact value is determined in the analysis.
% We denote $\mathbb{M} = \{M_1, M_2\}$.

Now, we consider a subset of algorithms $\mathfrak{A}' \subset \mathfrak{A}$.
Each algorithm $A\in\mathfrak{A}'$ that consumes $T$ samples from $c^1\in\mathcal{C}^1$ outputs a value function that takes the same value for different $(s,a)$s, i.e., $Q_T^A(c,s,a) = Q_T^A(c,s',a') =: \mathbb{Q}_T^A(c), \forall s,a,s',a'$. 
Then, we can obtain the following conclusion by replacing $\mathcal{S}\times\mathcal{A}$ with $\mathcal{C}$ in Lemma 18 in \cite{azar2013minimax}:
\begin{lemma}
\textit{
For $\delta \in (0,1/2)$ and any algorithm $A\in\mathfrak{A}'$ using a total number of context transition samples less than $T=c_1 \frac{|\mathcal{C}|}{(1-\gamma)^3 \epsilon^2} \log ( c_2 |\mathcal{C}|/\delta )$, there exists $M_m\in\mathbb{M}$ such that 
$$
\mathbb{P}_m (\| \mathbb{Q}^*_{M_m} - \mathbb{Q}^A_T \|_\infty > \epsilon) > \delta,
$$
where $\mathbb{P}_m$ is the probability under the model $M_m$ and $c_1, c_2$ are positive constants.
}
\end{lemma}

At last, we extend the conclusion to $\mathfrak{A}$ with the following lemma.
\begin{lemma}
\textit{
For any algorithm $A\in \mathfrak{A}$ that outputs $Q^A \in \mathbb{R}^{\mathcal{C}\times\mathcal{S}\times\mathcal{A}}$, we can always find an algorithm $A'\in\mathfrak{A}'$ such that 
$$
\| Q^*_M - Q^A \|_\infty \ge \| \mathbb{Q}^*_M - \mathbb{Q}^{A'} \|_\infty
$$
}
\end{lemma}
Actually, we can construct an algorithm $A'\in\mathfrak{A}'$ for each $A\in\mathfrak{A}$ by wrapping the output of $A$ as follows: $\mathbb{Q}^{A'}(c) := Q^A(c,s_0, a_0)$ for arbitrary fixed $s_0\in\mathcal{S}, a_0\in\mathcal{A}$.
\end{proof}

\textbf{Discussion.}
In the class of constructed ORDCs, we can categorize the contexts into six groups, three of which are the contexts $c^0\in\mathcal{C}^0$, $c^1\in\mathcal{C}^1$ and $c^2\in\mathcal{C}^2$ corresponding to $p_M=p$ and the other three corresponds to $p_M=p+\alpha$.
Aggregating the contexts into these six groups does not bring any loss in representing the optimal policy or value function.
In fact, it is possible to get rid of the $|\mathcal{C}|$ dependence in the sample complexity lower bound if the category of each context is known which is illustrated in Theorem \ref{theorem:upper_bound}.

==> inputs/app_proof2.tex <==
In the following proof, we use the lower case $p$ to represent the transition probability and the upper case $P$ to represent the corresponding matrix form, which is slightly different from the notation in the main text.
With access to $\phi$, the underlying transition model can be written as $p(x',s'|x,s,a) = p_x(x'|x) p_s(s'|x,s,a)$.
With a generative model, we can collect $N$ context transition samples from the context that corresponds to each latent context $x\in\mathcal{X}$.
Therefore, we consume a total number of $N|\mathcal{X}|$ samples.
Our algorithm estimates $p_x$ with these samples as follows: 
$\hat{p}_x(x'|x) = \text{count}(x,x') / \text{count}(x)$,
where $\text{count}(x,x')$ is the number of transitions from $x$ to $x'$ in the samples and $\text{count}(x)$ is the number of transitions starting from $x$ in the samples.

We denote $\hat{p}(x',s'|x,s,a) = \hat{p}_x(x'|x) p_s(s'|x,s,a)$ and the matrix form as $\hat{P}\in\mathbb{R}^{ |\mathcal{X}||\mathcal{S}||\mathcal{A}| \times |\mathcal{X}||\mathcal{S}| }$.
We can link the estimation error of $\hat{p}_x$ to that of $\hat{p}$ with the following lemma:
\begin{lemma}
\label{lemma:link}
\textit{
For any $x\in\mathcal{X}, s\in\mathcal{S}, a\in\mathcal{A}$, we have
$$
\| p(\cdot|x,s,a) - \hat{p}(\cdot|x,s,a) \|_1 = \| p_x(\cdot| x) - \hat{p}_x(\cdot|x) \|_1
$$
}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:link}]
$$
\begin{aligned}
& \| p(\cdot|x,s,a) - \hat{p}(\cdot|x,s,a) \|_1 \\
= & \sum_{x',s'} |p(x',s'|x,s,a) - \hat{p}(x',s'|x,s,a)|  \\
= & \sum_{x',s'} |p_x(x'|x) p_s(s'|x,s,a) - \hat{p}_x(x'|x) p_s(s'|x,s,a) |  \\
= & \sum_{x',s'} |p_x(x'|x) - \hat{p}_x(x'|x) | p_s(s'|x,s,a)  \\
= & \Big( \sum_{x'} |p_x(x'|x) - \hat{p}_x(x'|x) | \Big) \Big( \sum_{s'} p_s(s'|x,s,a) \Big)  \\
= & \| p_x(\cdot| x) - \hat{p}_x(\cdot|x) \|_1
\end{aligned}
$$
\end{proof}

Next, we introduce several lemmas for MDP. 
Notice that they also apply to our setting by treating the state in MDP as $(x,s)$ in the ORDC model.
\begin{lemma}[Lemma 2.2 in \cite{agarwal2019reinforcement}]
\label{lemma:22}
$$
Q^\pi - \hat{Q}^\pi = \gamma (I - \gamma \hat{P}^\pi)^{-1} (P - \hat{P}) V^\pi, \forall \pi
$$
\end{lemma}
\begin{lemma}[Lemma 2.3 in \cite{agarwal2019reinforcement}]
\label{lemma:23}
\textit{
For any policy $\pi$, and vector $v\in\mathbb{R}^{|\mathcal{X}||\mathcal{S}||\mathcal{A}|}$, we have
$$
\| (I - \gamma P^\pi)^{-1} v \|_\infty \le \|v\|_\infty / (1-\gamma)
$$
}
\end{lemma}
\begin{lemma}[Lemma A.8 in \cite{agarwal2019reinforcement}]
\label{lemma:A8}
\textit{
Let $z$ be a discrete random variable that takes values in $\{1, \cdots, d\}$ distributed according to $q\in\Delta^d$ with $q_i = Pr(z=i)$. 
Assume we have $N$ iid samples, and the empirical estimate $\hat{q}\in\Delta^d$ with $\hat{q}_i = \sum_{i=1}^N {\bf 1}[z_i=i] / N$.
For some constant $c>0$ and w.p. at least $1-\delta$, we have
$$
\| q - \hat{q} \|_1 \le c \sqrt{\dfrac{d \log(1/\delta)}{N}}.
$$
}
\end{lemma}

\begin{proof}[Proof of Theorem \ref{theorem:upper_bound}]
For any policy $\pi$, we have
$$
\begin{aligned}
& \| Q^\pi - \hat{Q}^\pi \|_\infty \\
= & \| \gamma (I - \gamma \hat{P}^\pi)^{-1} (P - \hat{P}) V^\pi \|_\infty \\
\le & \frac{\gamma}{1-\gamma}  \| (P - \hat{P}) V^\pi \|_\infty \\
\le & \frac{\gamma}{1-\gamma} \Big( \max_{x,s,a} \| p(\cdot|x,s,a) - \hat{p} (\cdot|x,s,a) \|_1  \Big)  \| V^\pi \|_\infty \\
= & \frac{\gamma}{1-\gamma} \Big( \max_{x} \| p_x(\cdot|x) - \hat{p}_x (\cdot|x) \|_1  \Big)  \| V^\pi \|_\infty \\
\le & \frac{\gamma}{(1-\gamma)^2} \Big( \max_{x} \| p_x(\cdot|x) - \hat{p}_x (\cdot|x) \|_1  \Big) \\
\le & c \frac{\gamma}{(1-\gamma)^2} \sqrt{\dfrac{|\mathcal{X}| \log(|\mathcal{X}|/\delta)}{N}} \quad \text{w.p. at least } 1-\delta. \\
\end{aligned}
$$
The first line uses Lemma \ref{lemma:22}. 
The second line uses Lemma \ref{lemma:23}.
The third line uses Holder's inequality.
The fourth line uses Lemma \ref{lemma:link}.
The fifth line uses Assumption \ref{assumption:MDP_regularity}.
The sixth line uses Lemma \ref{lemma:A8} with a union bound.
Equivalently, with $|\mathcal{X}| N = \dfrac{c^2 \gamma^2}{(1-\gamma)^4} \dfrac{|\mathcal{X}|^2 \log(|\mathcal{X}|/\delta)}{\epsilon^2}$ samples, we have $\| Q^\pi - \hat{Q}^\pi \|_\infty \le \epsilon$ w.p. at least $1-\delta$.

Then, for all $(x,s,a)\in\mathcal{X}\times\mathcal{S}\times\mathcal{A}$, we have
$$
\begin{aligned}
& |Q^*(x,s,a) - \hat{Q}^*(x,s,a)| \\
= & |\sup_\pi Q^\pi(x,s,a) - \sup_\pi \hat{Q}^\pi(x,s,a) | \\
\le & \sup_\pi |Q^\pi(x,s,a) - \hat{Q}^\pi(x,s,a)| \\
\le & \epsilon,
\end{aligned}
$$
which completes the proof.
\end{proof}

\textbf{An illustrative example.}
In addition to the proof, we also provide an illustrative view on how context aggregation can help generalization.
We consider a policy evaluation setting where we aim to estimate the value function for some context.
We will later show that, by aggregating the context properly, we can obtain a more accurate estimate of the value.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{inputs/fig_appendix.png}
    \caption{
    a) When a resettable environment is available, we can estimate $Q(c,s,a)$ accurately with the returns calculated based on fictitious context sequences (the gray lines).
    However, in real scenarios where fictitious context sequences cannot be obtained, we can only use the expected return calculated on few training sequences (the blue line) as the estimate which suffers from a large variance.
    b) When resorting to a mapping between the high-dimensional context and the latent context, we can obtain a better estimate by averaging over the returns calculated based on similar sequences (the orange lines). 
    }
    \label{fig:theorem2_illustration}
\end{figure}

Let us consider to estimate a value function $Q(c,s,a)$ for some $(c, s, a)\in\mathcal{C}\times\mathcal{S}\times\mathcal{A}$.
We illustrate the procedure under the simplified trade execution task (described in Section \ref{sec:toy_example}) in Figure \ref{fig:theorem2_illustration}.

When it is possible to reset the environment to $(c,s)$ and then take the action $a$ to rerun unlimited number of times, an accurate estimation of $Q(c,s,a)$ is $\hat{Q}'(c,s,a) = \frac{1}{N} (R'_1 + R'_2 + R'_3 + R'_4 + \cdots)$, where $R'_i$ is the cumulative return from $(c,s,a)$ in the $i$-th run (cf. the gray dashed lines in Figure \ref{fig:theorem2_illustration}a) and $N$ is the total number of runs.
When the number of samples is sufficient, $\hat{Q}'(c,s,a)$ approaches the true value $Q(c,s,a)$.

However, a resettable environment is not provided in most realistic scenarios, and therefore it is hard to obtain $R'$s.
For example, in the trade execution task, it is hard to reset to a specific market context and perform a counterfactual simulation on the complex market dynamics.
Without context aggregation (via either implicit function approximation or explicit context encoder), a straightforward way to estimate $Q(c,s,a)$ is to use the sample mean.
Suppose the context $c$ only appears once in the dataset (which is quite common when the context is high-dimensional).
In this scenario, the best estimate should be $\hat{Q}_1(c,s,a) = R_0$, where $R_0$ is the expected cumulative return calculated based on the only future context sequence (cf. the blue dashed lines in Figure \ref{fig:theorem2_illustration}a).
Notice that $\hat{Q}'(c,s,a)$ is calculated based on multiple context sequences but $\hat{Q}_1(c,s,a)$ is based on only one context sequence provided in the dataset.
Accordingly, $\hat{Q}_1(c,s,a)$ can suffer from a large variance.

An alternative method is to resort to the mapping between the high-dimensional context and the compact latent context.
When such a mapping is known, we can select the contexts that share a similar latent context to the interested context $c$ in the dataset (cf. the orange lines in Figure \ref{fig:theorem2_illustration}b).
Then, we can estimate the value function using $\hat{Q}_2(c,s,a) = \frac{1}{M} (R_0 + R_1 + R_2 + R_3 + R_4 + \cdots)$.
This estimate is the average of the returns collected based on multiple context sequences.
If these context sequences resemble the fictitious sequences starting from $(c,s,a)$ (cf. the gray dashed lines in Figure \ref{fig:theorem2_illustration}a),
we can consider $R_i\approx R'_i$ and therefore
$\hat{Q}_2(c,s,a)$ is an accurate estimate with reduced variance compared with $\hat{Q}_1$.

\iffalse

Based on the observation in the previous simplified trade execution task, we first introduce our motivation for a generalizable algorithm.
Then, we design an algorithm that is based on several hand-crafted target features for the real trade execution task.
Next, we propose an end-to-end algorithm that does not require any prior knowledge.

\textbf{Policy Evaluation}
In ORDC, the agent may overfit to the limited context sequences in the dataset.
We observe that, by resolving to a context encoding function $\phi:\mathcal{C} \to \mathcal{X}$ that maps the high-dimensional context into the latent context, we can obtain a more generalizable Q function.
Given a policy $\pi$, we learn a tabular Q function $q: \mathcal{X}\times\mathcal{S}\times\mathcal{A} \to \mathbb{R}$ by optimizing
\begin{equation}
    \min_q \frac{1}{N} \sum_{i=1}^N \Big( q(\phi(c_i), s_i, a_i) - \hat{Q}^\pi(c_i, s_i, a_i) \Big)^2,
\end{equation}
where $N$ is the number of training samples.
The corresponding solution is 
\begin{equation}
\begin{aligned}
    & q(x_t,s_t,a_t) = \\
    % & \frac{1}{M_{x_t}} \sum_{j=1}^{M_{x_t}} \frac{1}{N(c_j)} \sum_{i=1}^{N(c_j)} [R(c_j, s_t, a_t, \epsilon_c^{(j)}, \epsilon_c^{(i)}, \epsilon_\pi^{(i)})], 
    & \sum_{c\in\mathcal{D}} I(\phi(c)=x_t) \hat{Q}^\pi(c,s_t,a_t) / \Big[ \sum_{c\in\mathcal{D}} I(\phi(c)=x_t) \Big]
\end{aligned}
\end{equation}
where $\mathcal{D}$ is the offline context dataset.
By averaging over the contexts that share the same latent context, this estimator has smaller variance and avoid overfitting to the only context sequence in the dataset.

\subsection{Why generalization is difficult?}

Next, we explain why generalization is hard in the ORDC setting.
Here, we assume the latent context space $\mathcal{X}$ is discrete, and each context $c\in\mathcal{C}$ uniquely determines its generating latent context $x\in\mathcal{X}$ (i.e., block structure).

\textbf{Policy Evaluation} We consider the value-based RL method whose core is to estimate the Q function with samples collected from the simulator based on historical context data. 
Given a policy $\pi$, we aim to estimate
\begin{equation}
Q^\pi(c_t, s_t, a_t) = \mathbb{E}_{\epsilon_c} \mathbb{E}_{\epsilon_e, \epsilon_\pi}
[R(c_t, s_t, a_t, \epsilon_c, \epsilon_e, \epsilon_\pi)]
% [R({\bf s}_{t:T}, {\bf a}_{t:T}, {\bf c}_{t:T})],
\end{equation}
where $\epsilon_c, \epsilon_e$ and $\epsilon_\pi$ denote the randomness in context dynamics (i.e., in $s_{\tau-1} \to s_{\tau}$ and $s_{\tau} \to c_{\tau}, \forall \tau \in[t+1, T]$), in the environment (i.e., in state dynamics and the reward function), and in action selection.
The above randomness determines a complete trajectory and therefore the return after the $t$-th time step which is denoted as $R(c_t, s_t, a_t, \epsilon_c, \epsilon_e, \epsilon_\pi)$.
% $R$ is the cumulative reward when the state and action sequences are given.
% are calculated over all the possible action sequences sampled from the policy $\pi$, and $R$ is the cumulative reward when the state and action sequences are given\footnote{For ease of notation, we omit the randomness in state transitions and the reward function which should be averaged over in the second expectation.}.
While the expectation over $\epsilon_e$ and $\epsilon_\pi$ can be estimated with samples collected from the simulator, 
the expectation over $\epsilon_c$ cannot be accurately estimated due to limited context sequences provided in offline dataset.
For example, we consider the scenario where each context only appears once in the dataset which is common since the context is high-dimensional and the dataset is limited.
Therefore, the estimated Q value becomes
\begin{equation}
\hat{Q}^\pi(c_t, s_t, a_t) = \frac{1}{N(c_t)} \sum_{i=1}^{N(c_t)} [R(c_t, s_t, a_t, {\epsilon}_c^{(0)}, \epsilon_e^{(i)}, \epsilon_\pi^{(i)})],
\end{equation}
where $\epsilon_c^{(0)}$ indicates the only context sequence containing $c_t$ in the dataset, and $N(c)$ is the number of collected trajectory that contains $c$.
When the agent is trained with infinite number of samples collected from the simulator, the estimated Q value becomes $\mathbb{E}_{\epsilon_e,\epsilon_\pi}[R(c_t, s_t, a_t, \epsilon_c^{(0)}, \epsilon_e, \epsilon_\pi]$.
The estimated value function is prone to overfit to that context sequence.
For example, the agent may memorize the highest price in that context sequence and learn an aggressive policy that liquidates all the stocks on that price.
Indeed, the function approximation of neural networks may alleviate data scarcity of context sequences, but we observe overfitting in deep models empirically (see the next subsection).

\fi

==> inputs/app_simulator.tex <==
\textbf{Dataset.}
Compared with the simulators based on the preset stochastic process \cite{daberius2019deep} or a collection of preset interactive agents \cite{byrd2019abides}, the simulator driven by real market data can capture the complex market more accurately \cite{vyetrenko2020get}.
Moreover, compared with the previous work where the simulator is based on bar-level data, our simulator relies on the LOB-level data of the market which records an LOB snapshot every 3 seconds.
With finer-grained data, we are able to learn more practical trading agents.
For example, we can evaluate how an agent that trades using only MOs suffers from a large trading cost, which is the scheme adopted in many existing papers \cite{fang2021universal}.
The interested time period of trade execution tasks in the industry is typically from 10 to 120 minutes, which is configurable in our simulator.
% For higher fidelity, we extract information from the simulation is carried our snapshot by snapshot
% To avoid a long planning horizon, the agent can interact with our simulator in a lower frequency (one minute per step in our experiment), but the simulation is carried out snapshot by snapshot for accuracy.
Our simulator is based on the dataset that records an LOB snapshot every 3 seconds from the real market.
The time period of trade execution tasks in our experiments is set to 30 minutes.
To avoid a long planning horizon, the agent interacts with the simulator at a lower frequency (i.e., one minute per step).
Nevertheless, simulation is carried out snapshot by snapshot for higher accuracy.

\textbf{Observations.}
The observation in our simulator consists of the private variable (i.e., the state) and the market variable (i.e., the context).
The private variable consists of the remaining time and executed quantity.
The market variable can be the stacked features (including order-book-related features, technical indicators, raw snapshots, etc.) over several past steps. 
Our simulator implements a wide range of features including the features that appear in the previous papers as far as we know.
For different designs on the observations space, the agent can choose from these features.
To eliminate the differences in the features on different stocks,
the simulator normalizes the features as follows:
The price (or the feature whose dimension is price) is normalized using z-score with the open price on that trading day as the mean and the volatility on the previous trading day as the standard deviation.
The volume (or the feature whose dimension is volume) is normalized by dividing by the total volume of the last trading day.
In specific algorithms, we may perform another normalization on these features to fit them into a proper value range.

% The observation in our simulator consists of the market variables (context) and the private variables (state). 
% The market variables includes order-book related features, technical indicators, and are stacked over several past steps.
% Our simulator implements a wide range of features that appear in previous papers to choose from.
% The private variables consist of the remaining time and executed quantity.
% \blue{Normalization.}

% encode the information of the market (such as the price and volume) and the private variables include the remaining time and executed quantity.
% Different methods use different variables as the market variables such as order-book related features \cite{nevmyvaka2006reinforcement}, technical indicators \cite{ning2018double} or a stack of features of several past steps \cite{fang2021universal}.
% Our simulator implements a wide range of hand-crafted features and can easily generate different forms of observation variables through a configuration file.
% all the state variables in the previous papers as far as we know.

\textbf{Actions.}
On each time step, our simulator receives a list of orders, each of which can be an MO or LO that specifies the direction, the quantity, and the price (only for LO).
On top of this, we provide a series of wrappers to fit different designs on the action space (e.g., discrete/continuous/combinatorial action spaces).
% If the price is lower than the best bid price, the order will be executed as an MO. 
Our simulator will provide the best possible execution for each order.
For example, if the quoted price is lower than some bid price level, the simulator will automatically place an MO to fill the outstanding bid orders whose prices are higher than the quoted price, and an LO for the remaining quantity.
In our algorithms, the agent places an order on each step by choosing a quoted volume and a quoted price from discretized sets.
The quoted volume is selected from $\{\frac{1}{2}\text{TWAP}, \text{TWAP}, \frac{3}{2}\text{TWAP}, 2 \text{TWAP} \}$ where TWAP is the volume executed on each step by a TWAP strategy (i.e., selling an equal amount on each step).
The quoted price is specified by a price difference w.r.t. the best ask price. 
If the quoted price is lower than the best bid price, the agent actually places an MO; otherwise, it is an LO.
Outstanding orders at the end of each step will be withdrawn.
% However, different models use different action spaces such as placing orders with discrete prices with fixed quantity, only MOs with varying quantities, or even a combination of LOs and MOs \cite{karpe2020multi}.
% In our simulator, we provide a series of wrappers to fit different designs on the action space.

\textbf{Reward.}
The reward function may consist of a basic revenue term (e.g., negative trading cost or average execution price) and several regularization terms (e.g., approximating the permanent market impact or enforcing a TWAP-like strategy).
The revenue term reflects the overall objective of trade execution that minimizes the trading cost or the average execution price for a sell program.
Moreover, various of regularizers are adopted to model the permanent market impact or the prior knowledge of a good execution program (e.g., enforcing a TWAP-like program).
Our simulator provides various choices on the reward function design and can benchmark different designs with a uniform set of metrics (such as the trading cost or implementation shortfall \cite{perold1988implementation}).
In our algorithms, the reward function consists of a revenue term $r_1$ and a regularization term $r_2$, i.e., $r_t= r_1 + \beta r_2$ where $\beta$ is a coefficient.
The revenue term is $r_1 = n_t \bar{p}_t$ where
$n_t$ is the executed volume in the last step, and $\bar{p}_t$ is the corresponding average execution price.
The regularization term is $r_2 =  (v_t - v_{t,\text{TWAP}})^2$ where $v_t$ is the remaining inventory, and $v_{t,\text{TWAP}}$ is the remaining inventory if we follow the TWAP strategy.

% Although different algorithms use different reward functions, they are evaluated using a uniform set of  metrics.
% The basic reward function reflects the overall objective of trade execution which minimizes the trading cost or the average execution price for a sell program.
% Moreover, various of regularizers are adopted to model permanent market impact or the prior knowledge of a good execution program (e.g., enforcing a TWAP-like program).
% Our simulator provides various choices on the reward function design and can benchmark different design with a uniform set of metrics (such as trading cost or implementation shortfall \cite{perold1988implementation}).

\textbf{Transition dynamics.}
Given a list of orders on the $t$-th time step, our simulator will determine the reward and the state on the next time step.
For MOs, we consider the temporary market impact and the time delay.
For example, when the decision of the agent is based on observation generated on time $\tau$, the execution of an MO is based on the snapshot on time $\tau+\Delta\tau$ where $\Delta\tau$ is a preset time delay.
Typically, we use $\Delta\tau=3s$.
For LOs, we determine whether the order can be executed snapshot by snapshot till the ($t+1$)-th time step.
If the highest market price (i.e., a transaction occurs on this price) in one snapshot exceeds the price quoted in the LO, we consider the order is fully executed.
If the highest market price exactly equals the quoted price, the order may be partially filled and the ratio is calculated by reconstructing the transactions between snapshots.
However, considering that 1) the quantity may be too large to be fully executed or 2) the LO may be at the end of the queue of the quoted price level, we impose additional trading limits on the above matching mechanism to encourage conservative simulation.

\textbf{Discussion.}
To improve fidelity, our simulator considers the temporary market impact of MOs, the time delay, and determines the execution of LOs based on reconstructing the transactions between snapshots.
However, there are still components that we do not consider.
First, the permanent market impact is the change of the equilibrium price during at least our planning horizon when we place an order.
Here, we assume the permanent market impact is linear w.r.t. the order quantity and therefore considering this factor does not change the optimal solution of our strategy \cite{almgren2001optimal}.
Then, MOs in our simulation not only change the current LOB but also the LOB of the next time step, possibly resulting in degenerated fidelity.
Therefore, we also rely on the assumption that the limit orders are resilient within a short period of time (which should be smaller or comparable to the time interval between two simulation steps).
Fortunately, this is verified by empirical studies such as \cite{degryse2005aggressive,cummings2010further,gomber2015liquidity}.


==> inputs/sec_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
\iffalse
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{We use CC-BY-NC-ND.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
\fi
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Appendix \ref{app:execution_experiments}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix \ref{app:execution_experiments}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We uploaded our code in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{app:execution_experiments}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We reported standard deviations.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{app:execution_experiments}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> inputs/tab_interprebility.tex <==
\begin{table}[t]
    \centering
    \small

\begin{tabular}{lrr}
\toprule
Predicted Statistics &   Price &  Volume \\
\midrule
Avg future twap - current twap &  4.5296 & -0.0420 \\
Max future twap - current twap &  1.3932 & -0.1761 \\
Min future twap - current twap & -1.0587 &  0.2978 \\
Twap volatility                &  1.2871 & -0.4335 \\
Avg future sprd - current sprd & -0.0944 &  0.0879 \\
Max future sprd - current sprd &  1.8254 & -0.2629 \\
Min future sprd - current sprd & -1.2859 &  0.1579 \\
Sprd volatility                &  6.2039 & -0.6810 \\
\bottomrule
\end{tabular}

    \caption{The impact of predicted statistics on the agent's action in CASH (based on PPO).}
    \label{tab:interpretability}
\end{table}
